ReRec: Reasoning-Augmented LLM-based Recommendation Assistant via Reinforcement Fine-tuning

With the rise of LLMs, there is an increasing need for intelligent recommendation assistants that can handle complex queries and provide personalized, reasoning-driven recommendations. LLM-based recommenders show potential but face challenges in multi-step reasoning, underscoring the need for reasoning-augmented systems. To address this gap, we propose ReRec, a novel reinforcement fine-tuning (RFT) framework designed to improve LLM reasoning in complex recommendation tasks. Our framework introduces three key components: (1) Dual-Graph Enhanced Reward Shaping, integrating recommendation metrics like NDCG@K with Query Alignment and Preference Alignment Scores to provide fine-grained reward signals for LLM optimization; (2) Reasoning-aware Advantage Estimation, which decomposes LLM outputs into reasoning segments and penalizes incorrect steps to enhance reasoning of recommendation; and (3) Online Curriculum Scheduler, dynamically assess query difficulty and organize training curriculum to ensure stable learning during RFT. Experiments demonstrate that ReRec outperforms state-of-the-art baselines and preserves core abilities like instruction-following and general knowledge. Our codes are available at https://github.com/jiani-huang/ReRec.

==> Tables/2-Notations.tex <==

\begin{table}[t]
\centering
\caption{Main symbols used in this paper.}
\small % Set the font size for the table
\begin{tabular}{|c|l|}
\hline
\textbf{Symbol} & \textbf{Description} \\ \hline
$q$ & The query that the user is looking for recommendations \\ \hline
$gt$ & The ground truth item that satisfies the user query \\ \hline
$\pi_\theta$ & The LLM policy model \\ \hline
$G$ & The size of the group of outputs for each $q$ during rollout \\ \hline
$o_i$ & The $i$-th output in a set of outputs \\ \hline
$t$ & The $t$-th token of output \\ \hline
$p_i$ & The predicted item which can be extracted from output $o_i$ \\ \hline
$S_i$ & Reasoning steps of output $o_i$ \\ \hline
$\mathcal{R}$ & Reward model that generates rewards for outputs \\ \hline
$r_i$ & Reward of output $o_i$ \\ \hline
$A_{it}$ & Advantage of token $t$ in output $i$ \\  \hline
\end{tabular}
\label{tab:notations}
\end{table}


==> Tables/2-Preliminaries.tex <==
\section{Preliminaries}
% \remove{In this section, we begin by introducing the key notations used throughout the paper. We then define our recommendation task, followed by an overview of the RFT process that optimize LLMs for recommendation tasks.}


% \textsc{Notations.} Table~\ref{tab:notations} outlines the main symbols used in this paper. 
% \input{Tables/2-Notations}

\textbf{Problem Statement.}
% \textbf{\expander\capitalisewords\expand{\ourtask.}}
In real-world scenarios, users often express their preferences through rich, multi-faceted natural language queries. 
For example, a user may ask, "\emph{I remember a sci-fi movie where the hero chased bad guys on a hoverboard with a time machine. I really liked the male lead. Can you recommend more movies with him?}" 
We consider such queries to be complex queries, as they go beyond simple keyword matching or attribute filtering, requiring the \textbf{recommendation assistant} to perform \textbf{multi-step reasoning} for understanding multiple aspects of the user's intent.
Mathematically, given a user's query $q$, the objective of the LLM-based recommendation assistant $\pi_\theta$ is to generate a response $o$ that encompasses both the reasoning process and a specific recommended item $p$. 
Specifically, the reasoning process should clarify why the assistant selects a particular item $p$ and why other potential items were not chosen. 
Formally, the process is defined as 
$\pi_\theta(q) = o$. 

\noindent
\textbf{Reinforcement Fine-tuning (RFT) for Recommendation.} 
During training, to enhance the reasoning and recommendation capability of the LLM-based recommendation assistant $\pi_\theta(q)$, reinforcement fine-tuning~\cite{wang2025re2llm,wang2025large} is usually employed to optimize the policy of the assistant $\pi_\theta(q)$.  
Generally, given the input query $q$, the assistant will generate corresponding responses $\{o_1, o_2, ...,o_G\}$ based on the learned policy $\pi_\theta$. 
After that, the generated responses are evaluated by the \textit{Reward Model} to assign reward scores $r_i$, and such scores are further employed to compute advantages $A_i$. 
These advantages indicate which responses are better, guiding the LLM policy model to optimize toward better outputs. 
The specific components are detailed as follows:
% \vspace{-0.5em}
\begin{itemize}[leftmargin=*]
    \item \textit{Reward Model ($\mathcal{R}$).} For each generated output $o_i$, a predefined Reward Model $\mathcal{R}$ computes a corresponding reward value $r_i$, expressed as $ r_i=\mathcal{R}(o_i, gt) $ for each $ o_i $ with $ gt $ as the ground truth. 
    In the context of LLM-based recommendation, Normalized Discounted Cumulative Gain (NDCG)~\cite{jarvelin2002cumulated} or Recall~\cite{gunawardana2012evaluating} can be utilized as a reward model to evaluate output quality. 
    
    \item \textit{Advantage Estimation ($A$).} Existing research has demonstrated that directly using rewards for gradient estimation in policy optimization typically leads to high variance and unstable updates, as rewards are often noisy and lack a reference point for comparison~\cite{schulman2017proximal}. 
    Therefore, recent studies introduce the advantage value, which compares the actual reward received to the expected reward the policy would typically achieve in that state~\cite{arulkumaran2017deep,mehta2020state}. 
    If the reward is higher than expected, the advantage is positive, encouraging the policy to favor similar actions in the future. 
    For example, in popular sampling-based advantage estimation methods~\cite{ahmadian2024back,shao2024deepseekmath,hu2025reinforce++}, 
    for a given query $q$, the LLM policy model samples multiple responses $\{o_1, o_2, ...,o_G\}$, each representing a trajectory where each token is an action taken by the model.
    Subsequently, an advantage value $A_{i,t}$ is calculated for every token in each response to identify preferred trajectories or actions.  
    For instance, in Group Relative Policy Optimization (GRPO)~\cite{shao2024deepseekmath}, the advantages can be calculated as $A_{i,t} = \frac{r_i - \operatorname{mean}(\textbf{r})}{\operatorname{std}(\textbf{r})}$.
    % \begin{align}
    %     A_{i,t} = \frac{r_i - \operatorname{mean}(\textbf{r})}{\operatorname{std}(\textbf{r})}.
    % \end{align}

    \item \textit{Training Objective ($\mathcal{J}(\theta)$).} Based on the computed advantages, the policy of LLM-based recommendation assistant is usually optimized by maximizing the following objective~\cite{shao2024deepseekmath}:
    \begin{equation}
        \begin{aligned}
        & \mathcal{J}(\theta) = \mathbb{E}_{(q,gt) \sim \mathcal{D}, \{o_i\}_{i=1}^G \sim \pi_{\theta_{\text{old}}}(\cdot \mid q)} = &  \\
        & \left[ \frac{1}{N} \sum_{i=1}^G \sum_{t=1}^{|o_i|} \min \left( h_{i,t}(\theta) A_{i,t},\text{clip} \left( h_{i,t}(\theta), c_{low}, c_{high}\right) A_{i,t} \right) \right],
        \label{eq:obj}            
        \end{aligned}
    \end{equation}

    \noindent
    where \( N = \sum_{i=1}^G |o_i| \), \( h_{i,t}(\theta) = \frac{\pi_\theta(o_{i,t} \mid q, o_{i,<t})}{\pi_{\theta_{\text{old}}}(o_{i,t} \mid q, o_{i,<t})} \), the \( \text{clip} \) function represents the clipped probability ratio, \( \varepsilon \) is a hyperparameter, and \( c_{low} = 1 - \varepsilon \), \( c_{high} = 1 + \varepsilon \). 
    % Table~\ref{tab:notations} outlines the main symbols used in this paper. 
    
\end{itemize}






% \input{Tables/2-Notations}


% \vspace{-1em}



==> Tables/RQ2-table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{The overall performance of baselines and \ourmodel on Query-and-History Setting}
  \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{cccc|ccc}
    \toprule
    \multicolumn{1}{c}{Model} & \multicolumn{3}{c|}{Movie}             & \multicolumn{3}{c}{Book} \\
          & \multicolumn{1}{c}{Explicit} & \multicolumn{1}{c}{Implict} & \multicolumn{1}{c|}{Misinformed} & \multicolumn{1}{c}{Explicit} & \multicolumn{1}{c}{Implict} & \multicolumn{1}{c}{Misinformed} \\
    \midrule
    \multicolumn{1}{c}{\textbf{\textit{LLM Backbone}}} &       &       &       &       &       & \\
    \multicolumn{1}{c}{Qwen-2.5-3B} & 0.217      &  0.130     &  0.090     & 0.426     & 0.394      & 0.314 \\
    % \multicolumn{1}{c}{Qwen-2.5-72B} &       &       &       &       &       & \\
    \multicolumn{1}{c}{GPT-4o} &       &       &       &       &       & \\
    \multicolumn{1}{c}{Deepseek-R1} &       &       &       &       &       & \\
    \midrule
    \multicolumn{1}{c}{\textbf{\textit{LLM-based CRS}}} &       &       &       &       &       & \\
    \multicolumn{1}{c}{InteRecAgent} &       &       &       &       &       & \\
    \multicolumn{1}{c}{CRAG} &       &       &       &       &       & \\
    \midrule
    \multicolumn{1}{c}{\textbf{\textit{Reasoning Model}}} &       &       &       &       &       & \\
    \multicolumn{1}{c}{GRPO} & 0.572    &   0.527    &  0.465      & 0.876      &  0.881     &  0.858\\
     \multicolumn{1}{c}{REINFORCE++} & 0.578  & 0.523 & 0.533 & 0.877 & 0.873 & 0.863 \\
     \multicolumn{1}{c}{RLOO} & 0.500 & 0.451  & 0.477 & 0.816  & 0.853  &    0.847  \\
    \multicolumn{1}{c}{\textbf{\ourmodel}} & 0.589 & 0.556 & 0.535 & 0.894 & 0.893  & 0.894 \\
    % imp. / best & & & & & & \\
    \bottomrule
    \end{tabular}%
}
  \label{tab:rq2}%
\end{table}%

% movie
% grpo: 30
% \ourmodel: 105

% book
% grpo: 20
% \ourmodel: 55

